A scalable deep learning approach for solving high-dimensional dynamic optimal transport

The dynamic formulation of optimal transport has attracted growing interests in scientific computing and machine learning, and its computation requires to solve a PDE-constrained optimization problem. The classical Eulerian discretization based approaches suffer from the curse of dimensionality, which arises from the approximation of high-dimensional velocity field. In this work, we propose a deep learning based method to solve the dynamic optimal transport in high dimensional space. Our method contains three main ingredients: a carefully designed representation of the velocity field, the discretization of the PDE constraint along the characteristics, and the computation of high dimensional integral by Monte Carlo method in each time step. Specifically, in the representation of the velocity field, we apply the classical nodal basis function in time and the deep neural networks in space domain with the H1-norm regularization. This technique promotes the regularity of the velocity field in both time and space such that the discretization along the characteristic remains to be stable during the training process. Extensive numerical examples have been conducted to test the proposed method. Compared to other solvers of optimal transport, our method could give more accurate results in high dimensional cases and has very good scalability with respect to dimension. Finally, we extend our method to more complicated cases such as crowd motion problem.

==> TheProposedMethod.tex <==
\section{The Proposed Method}\label{TheProposedMethod}

\subsection{Relaxation of Dynamical OT}
\iffalse
Consider the following general optimal control problem:
\begin{align*}
\min_{(\boldsymbol{v},\rho) \in V \times W} &\mathcal{F}(\boldsymbol{v},\rho)\\
s.t.~~~~ &\mathcal{A}(\boldsymbol{v},\rho) = 0.
\end{align*}
where $\boldsymbol{v}: \mathbb{R}^d \times [0,1] \longrightarrow \mathbb{R}^d$ is the vector field, $\rho: \mathbb{R}^d\times [0,1]\longrightarrow \mathbb{R} $ is the density distribution. $\mathcal{F}: V \times W \longrightarrow \mathbb{R}$ is the objective function.
$\mathcal{A}: V \times W \longrightarrow Z$ is an operator, the operator equation $\mathcal{A}(\boldsymbol{v},\rho) = 0$ represents a system of PDEs, and $V, W, Z$ are real generalized function spaces.

The dynamic MFP problem has the following optimization formulation:
\begin{align*}
\min _{\boldsymbol{v}, \rho} &\int_{0}^{1} \int_{\Omega} L(\rho(t, \boldsymbol{x}), \boldsymbol{v}(t, \boldsymbol{x})) \mathrm{d} \boldsymbol{x} \mathrm{d} t+\int_{0}^{1} \mathcal{Q}(\rho(t, \cdot)) \mathrm{d} t\\
s.t.\quad & \partial_{t} \rho(x,t)+\nabla _{\boldsymbol{x}} \cdot (\rho(x,t) \boldsymbol{v}(x,t)) =0\\
&\rho(x,0)=\rho_0(x),\rho(x,1)=\rho_1(x)
\end{align*}
By relaxing the given terminal density as an implicit condition regularized by a functional $\mathcal{P}$, one can retrieve a class of MFG as the following formulation:
\begin{align*}
\min _{\boldsymbol{v}, \rho} &\int_{0}^{1} \int_{\Omega} L(\rho(t, \boldsymbol{x}), \boldsymbol{v}(t, \boldsymbol{x})) \mathrm{d} \boldsymbol{x} \mathrm{d} t+\int_{0}^{1} \mathcal{Q}(\rho(t, \cdot)) \mathrm{d} t+ \mathcal{P}(\rho(1, \cdot))\\
s.t.\quad & \partial_{t} \rho(x,t)+\nabla _{\boldsymbol{x}} \cdot (\rho(x,t) \boldsymbol{v}(x,t)) =0\\
&\rho(x,0)=\rho_0(x)
\end{align*}

\fi


The dynamical formulation of optimal transport is actually a density optimal control problem. In addition,
$\mathcal{E}(\boldsymbol{v},\rho)$ defined in \eqref{dOT} denotes the kinetic energy (up to a factor $\frac{1}{2}$). We relax the given terminal density into an implicit condition by introducing a  Kullback–Leibler(KL) divergence penalty term:
\begin{align*}
\mathcal{P}(\rho)&:= \lambda \int_{\Omega}\rho(x,1)\log \frac{\rho(x,1)}{\rho_1(x)}
\mathrm{d}x
\end{align*}
$\mathcal{P}(\rho)$ is the KL divergence between $\rho(\cdot,1)$ and $\rho_{1}$ up to a sufficiently large positive constant $\lambda$, which is the penalty parameter.

From \eqref{opTt} we know that the characteristic of the optimal solution $T_{t}$ is a straight line connecting two points $x$ and $T(x)$,
In order to use the priori information, we introduce the Frobenius norm of the gradient of the velocity field as the regularization item $\mathcal{R} (\boldsymbol{v})$, i.e,
\begin{align*}
    \mathcal{R} (\boldsymbol{v}):= \alpha \int_{0}^{1}\int_{\Omega} |\nabla \boldsymbol{v}(x,t)|_{F}^{2} \mathrm{d}x
    \mathrm{d}t
\end{align*}
where $|*|_{F}$ denotes Frobenius norm.

By relaxing the terminal density as an implicit condition penalized by KL divergence term and introducing the regularization term, we can get the following optimal control formulation:
\begin{align}\label{objective}
\min_{(\boldsymbol{v},\rho) \in \mathcal{C}(\rho_0)}\mathcal{F}(\boldsymbol{v},\rho) = \mathcal{E}(\boldsymbol{v},\rho) + \mathcal{P}(\rho) + \mathcal{R}(\boldsymbol{v})
\end{align}
where $\mathcal{C}(\rho_0):=\{(\rho, \boldsymbol{v}): \partial_t \rho+\nabla\cdot (\rho \boldsymbol{v})=0, \rho(\cdot,0)=\rho_0\}$.
%By using the Kullback-Leibler divergence and $L_2$ penalty, it can be rewritten as
%\begin{align*}
% &\min_{\mathbf{v}}\int_{0}^1\int_{\Omega} | \mathbf{v}(x,t)|^2\rho(x,t)dxdt + \lambda_1 \int_{\Omega}\rho(x,1)\log \frac{\rho(x,1)}{\rho_1(x)}dx + \lambda_2 \int_{\Omega}( \rho(x,1)-\rho_1(x))^2 dx+ \alpha \mathcal{R} (\mathbf{v}),\\
% &s.t.~~~~ \partial_t \rho(x,t)+\nabla\cdot (\rho(x,t)\mathbf{v}(x,t))=0, t \in (0,1]\\
%&~~~~~~~~\rho(x,0)=\rho_0(x), x \in \Omega.
%\end{align*}

\subsection{Lagrangian Discretization}
In order to solve the high-dimensional optimal transport problems, we natually adopt the Lagrangian discretization method instead of the traditional mesh-based method. Because the Lagrangian discretization is a sampling method which can reduce memory usage for overcoming the curse of dimensionality.
Firstly, it is well-known that the continuity equation in $\mathcal{C}(\rho_0)$ can be approximately solved along the characteristics:
\begin{align}
&\frac{\mathrm{d}}{\mathrm{d}t}\mathbf{z}(x,t)=\boldsymbol{v}(\mathbf{z}(x,t),t),\mathbf{z}(x,0)=x,  \label{char}\\
&\frac{\mathrm{d}}{\mathrm{d}t}\rho(\mathbf{z}(x,t),t)=-\rho(\mathbf{z}(x,t),t)\nabla\cdot \boldsymbol{v}(\mathbf{z}(x,t),t),\rho(\mathbf{z}(x,0),0)=\rho_0(x). \label{rhos}
\end{align}

Together with the Lagrangian method \eqref{char} and \eqref{rhos}, this leads to an optimization problem with respect to the velocity filed $\boldsymbol{v}$, which we will model with a neural network.
In addition, we use Monte Carlo method for integration and suppose $x_1,x_2,...,x_r$ are samples drawn from $\mu_0$ (here $\mu_0$ are commonly uniform distribution or $\mu_0=\rho_0$), and $y_1,y_2,..,y_s$ are samples drawn from a uniform distribution whose density is $P_0$ to get the following semi-discretization version of optimal transport problem.
\begin{align}\label{prov} 
 \min_{\boldsymbol{v} }\overline{\mathcal{F}} (\boldsymbol{v},\rho) :=  \overline{\mathcal{E}} (\boldsymbol{v},\rho)  + 
 \overline{\mathcal{P}} (\rho) + \overline{\mathcal{R}} (\boldsymbol{v})
\end{align} 
where $\overline{\mathcal{E}} (\boldsymbol{v},\rho),  \overline{\mathcal{P}} (\rho)$ and $\overline{\mathcal{R}} (\boldsymbol{v})$ are the discretization versions of $\mathcal{E}(\boldsymbol{v},\rho), \mathcal{P}(\rho)$ and $\mathcal{R}(\boldsymbol{v})$ in the space direction respectively, i.e.,
\begin{align}
\overline{\mathcal{E}} (\boldsymbol{v},\rho)&:= \int_0^1 \sum_{i=1}^r w_i(t)|\boldsymbol{v}(\mathbf{z}(x_i,t),t)|^2 \mathrm{d}t \label{disE}\\
\overline{\mathcal{P}} (\rho)&:= {\lambda}\sum_{i=1}^r w_i(1) \log \frac{\rho(\mathbf{z}(x_i,1),1)}{\rho_1(\mathbf{z}(x_i,1))}\label{disP}\\
\overline{\mathcal{R}} (\boldsymbol{v})&:= \frac{\alpha}{s P_0}\int_0^1\sum_{j=1}^s|\nabla \boldsymbol{v}(y_j,t)|_F^2 \mathrm{d}t \label{disR}
\end{align}
and 
\begin{align*}
    w_i(t) = \frac{\rho(\mathbf{z}(x_i,t),t)}{\mu(\mathbf{z}(x_i,t),t)r}
\end{align*}
where $\rho(\mathbf{z}(x_i,t),t)$ and $\mu(\mathbf{z}(x_i,t),t)$ are the solution of \eqref{rhos} with different initial value $\rho_{0}(x_i)$ and $\mu_{0}(x_i)$ along the characteristics $\mathbf{z}(x_i,t)$. Then, \eqref{char} and \eqref{rhos} can be reformulated as the following constraints:
\begin{align}
 &\frac{\mathrm{d}}{\mathrm{d}t}\mathbf{z}(x_i,t)=\boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mathbf{z}(x_i,0)=x_i, ~x_i \sim \mu_0(x_{i}), \label{forwd1}\\
 &\frac{\mathrm{d}}{\mathrm{d}t}\rho(\mathbf{z}(x_i,t),t)=-\rho(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\rho(\mathbf{z}(x_i,0),0)=\rho_0(x_i),\label{forwd2}\\
 &\frac{\mathrm{d}}{\mathrm{d}t}\mu(\mathbf{z}(x_i,t),t)=-\mu(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mu(\mathbf{z}(x_i,0),0)=\mu_0(x_i).\label{forwd3}
 \end{align}
 
Note that for $\mu_0 = \rho_0$, the optimization problem \eqref{prov} with three constraints \eqref{forwd1}, \eqref{forwd2} and \eqref{forwd3} becomes a simplified problem with $w_i(t)=\frac{1}{r}, i = 1,...,r$ and only two ODE constraints \eqref{forwd1}, \eqref{forwd2} should be solved and one less equation than the original optimization problem. 
 
In summary, the problem becomes the following constrained optimization problem:
\begin{align}
    \min_{\boldsymbol{v} }\overline{\mathcal{F}} (\boldsymbol{v},\rho)
\end{align}
s.t.
\begin{equation}  
\left\{  
    \begin{aligned} 
 &\frac{\mathrm{d}}{\mathrm{d}t}\mathbf{z}(x_i,t)=\boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mathbf{z}(x_i,0)=x_i, ~x_i \sim \mu_0(x_{i})\\
 &\frac{\mathrm{d}}{\mathrm{d}t}\rho(\mathbf{z}(x_i,t),t)=-\rho(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\rho(\mathbf{z}(x_i,0),0)=\rho_0(x_i)\\
 &\frac{\mathrm{d}}{\mathrm{d}t}\mu(\mathbf{z}(x_i,t),t)=-\mu(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mu(\mathbf{z}(x_i,0),0)=\mu_0(x_i)  
\end{aligned}  
\right.  
\end{equation} 

 \subsection{Gradient Calculation}
In this paper we parameterize the velocity field $\boldsymbol{v}$ by using a neural network $\boldsymbol{v}(x,t;\theta)$, where $\theta$ denotes the trainable parameters. The structure of the neural network will be mentioned in the next section. Then, the original optimization problem for the velocity filed $\boldsymbol{v}$ \eqref{prov} can be changed into the current optimization problem with respect to the parameters $\theta$. Next, in order to calculate the gradient of the loss function with respect to $\theta$, we have adopt two different methods: the back propagation method and the adjoint state method, which correspond to the discrete-then-optimize and optimize-then-discrete, respectively. In Appendix \ref{appadsm} and \ref{AppCwBP}, we introduce the adjoint state method and compare it with the back propagation method in numerical experiments for the Gaussian problem. In this section, we will provide the calculation of the gradient by using the back propagation method since it achieves superior results at reduced computational costs. 

 \subsubsection{Back propagation}
 In the discrete-then-optimize method, backpropagation is realized by using automatic differentiation, which traverses the computational graph backward in time and is used commonly in
machine learning frameworks. Actually, the discretization of the forward propagation completely determines
this process.

Since \eqref{prov} is the semi-discretization objective function, we can simplify it as 
\begin{align}
\overline{\mathcal{F}} (\theta) = \int_0^1 f(t;\theta) \mathrm{d}t + 
\overline{\mathcal{P}} (\rho)
\label{semdis2}
\end{align}
where
\begin{align*}
f(t;\theta) = \sum_{i=1}^r w_i(t)|\boldsymbol{v}(\mathbf{z}(x_i,t),t;\theta)|^2 + \frac{\alpha}{s P_0}\sum_{j=1}^s|\nabla \boldsymbol{v}(y_j,t;\theta)|_F^2
\end{align*}
We use composite Simpson formula to discrete the semi-discretization objective function \eqref{semdis2}.
\begin{align*}
\int_{0}^{1} f(t) \mathrm{d}t & = \sum_{n=0}^{N-1} \int_{t_n}^{t_{n+1}} f(t) \mathrm{d}t
\approx \frac{h}{6}\sum_{n=0}^{N-1}[ f(t_{n})+4f(t_{n}+\frac{h}{2})+ f(t_{n+1})]
\end{align*}
where $h = \frac{1}{N}, t_{n} = nh, n = 0,\dotsc,N$.

Next, the computation of the gradients using the back propagation method follows three steps: forward pass, loss calculation and backward pass. We first perform the forward pass by using the fourth-order explicit Runge-Kutta scheme (RK4) to solve ODE constrains \eqref{forwd1}, \eqref{forwd2} and \eqref{forwd3}. Then, we can further adopt the Simpson formula to calculate the loss function $\overline{\mathcal{F}}(\theta)$. Finally,  during the backward pass, the automatic differentiation technique can be used to compute the gradients with respect to the network parameters $\frac{\partial \overline{\mathcal{F}}}{\partial \theta}$, which will be used to update $\theta$. The computational flow chart for calculating the gradients using the backpropagation method is shown in Fig.2.1.

\begin{figure}[h]
\begin{center}
\includegraphics[width=12cm]{images/BP2.png}
\caption{The illustration of the back propagation algorithm.}
\end{center}
\end{figure}

\iffalse
 \subsubsection{Adjoint state method}

 In adjoint state method, the gradients are computed by numerically solving the adjoint equation
\begin{proposition}
		The gradient of $\overline{\mathcal{F}} (\theta)$ is given by the following formula.
\begin{align*}
	\frac{\partial \overline{\mathcal{F}} (\theta)}{\partial
	\theta} = &
	\frac{1}{r}\sum_{i=1}^{r} \int_{0}^{1}[2\dfrac{\rho(\mathbf{z}_i(t),t)}{\mu(\mathbf{z}_i(t),t)}\boldsymbol{v}(\mathbf{z}_i(t),t)^{T}-U_i^T(t)]\boldsymbol{v}_{\theta}(\mathbf{z}_i(t),t;\theta)~\mathrm{d} t \\
	&+\frac{\alpha}{sP_{0}}\sum_{j=1}^{s}\int_{0}^{1}2\left \langle \nabla\boldsymbol{v}_{\theta}(y_{j},t;\theta),\nabla \boldsymbol{v}(y_{j},t)  \right \rangle  \mathrm{d} t
\end{align*}
Here we denote $\mathbf{z}(x_i,t)$ by $\mathbf{z}_i(t)$ for simplification. 
$\left \langle \cdot,\cdot  \right \rangle $ is defined as
\begin{align*}
    \left \langle A,B  \right \rangle = \sum_{i,j}A_{i,j}B_{i,j}
\end{align*}
$A,B$ is two matrices with the same size.
And
$U_i(t)$ is solution of the following ODEs
$$
\left\{
\begin{aligned}
\dfrac{\mathrm{d}U_i(t)}{\mathrm{d}t}&+\nabla^T\boldsymbol{v}(\mathbf{z}_i(t),t)U_i(t)=c_i(t) \\
U(1^-)&=-a_i
\end{aligned}
\right.
$$
where
\begin{align*}
a_i^T  =  [\frac{\lambda}{\mu}(\log{\frac{\rho}{\rho_1}}+1)\nabla\rho-
\frac{\lambda\rho}{\mu^2}\log{\frac{\rho}{\rho_1}}\nabla\mu-
\frac{\lambda\rho}{\mu \rho_1} \nabla\rho_1 ]
(\mathbf{z}_i(1),1)
\end{align*}
\begin{align*}
	c_i^T(t) & = [\frac{2\rho }{\mu}\boldsymbol{v}^T\nabla \boldsymbol{v}+ 
	\frac{|\boldsymbol{v}|^2}{\mu ^2}(\mu \nabla \rho -\rho \nabla \mu ) ](\mathbf{z}_i(t),t)
\end{align*}
\end{proposition}

The detailed proof of the above proposition is shown in the Appendix \ref{appadsm} \ref{AppCwBP}. 
For the adjoint state method, the computation of the gradients also follows three steps: forward pass, backward pass and gradient calculation, which are different from the back propagation method. Firstly, the forward pass is realized by using the fourth-order explicit Runge-Kutta scheme only to solve \eqref{forwd1} to get the activation throughout time $\mathbf{z}(t)$. Then, the terminal value condition of the adjoint ODE, $U_{t_N}=U(t=1)$, can be further computed by plugging in the values for $\mathbf{z}_{t_N}=\mathbf{z}(t=1)$. During the backward pass, we need to solve the adjoint ODE to compute $U(t)$ by using all activations $\mathbf{z}(t)$ and still the fourth-order explicit Runge-Kutta scheme. Finally, the gradient with respect to the network parameters $\frac{\partial \overline{\mathcal{F}}}{\partial \theta}$ can be computed by using $\mathbf{z}(t)$ and $U(t)$. The computational flow chart for calculating the gradients using the adjoint state method is shown in Fig.2.2.

It is worth to mention that in order to reduce the memory storage for all activations $\mathbf{z}(t)$, only the activation of the last state $\mathbf{z}(1)$ need to be saved in the forward pass, while the intermediate states $\mathbf{z}(t)$ can be recalculated through the backward pass.

\begin{figure}[h]
\begin{center}
\includegraphics[width=12cm]{images/Adjoint2.png}
\caption{The illustration of the adjoint state method.}
\end{center}
\end{figure}
\fi

\subsection{Neural Network Parameterization}
In order to solve high-dimensional op timal transport problem, we parameterize the velocity field by using a neural network, which can naturally lead to a mesh-free scheme and overcome the curse of dimensionality.
We now introduce our neural network parameterization of the velocity field.
In the following, we denote our model
as 
 \begin{align*}
 \boldsymbol{v}(x,t;\theta) = \sum_{i=0}^M\boldsymbol{v}_i(x;\theta)\phi_i(t),
 \end{align*}
 where $(x,t) \in \mathbb{R}^{d+1}$ is the input feature, $\theta$ is the network parameters and $\phi_i(t)$ is chosen as the nodal basis function in the time direction, i.e.,
\begin{align*}
\phi_i(t)=
\begin{cases}
0,&t\leq t_{i-1},\\
\frac{t-t_{i-1}}{t_i-t_{i-1}}=M(t-t_{i-1}),&t_{i-1}<t\leq t_i,\\
\frac{t_{i+1}-t}{t_{i+1}-t_{i}}=M(t_{i+1}-t),&t_{i}<t\leq t_{i+1},\\
0,&t> t_{i+1}.
\end{cases}
\end{align*}
and $M+1$ denotes the number of the basis function. Besides, $\boldsymbol{v}_i(x;\theta)$ is a two-layer neural network designed as $\mathbf{v}_i(x;\theta)=\sum_{l=1}^L[W_{2i}^{(l)}\sigma(W_{1i}^{(l)}x+b_{1i}^{(l)})+b_{2i}^{(l)}]$, $W_{1i}^{(l)} \in \mathbb{R}^{H \times d}$, $W_{2i}^{(l)} \in \mathbb{R}^{d \times H}$, $b_{1i}^{(l)} \in \mathbb{R}^{H}$, $b_{2i}^{(l)} \in \mathbb{R}^{d}$, the network parameters $\theta = \{W_{1i}^{(l)}, W_{2i}^{(l)}, b_{1i}^{(l)}, b_{2i}^{(l)}\}$, $L$ is the width of the network and $\sigma(x)=\tanh(x)$ is the activation function. 
The advantage of the design of our neural network architecture is to reduce the oscillations in the time direction because we use the piecewise linear function to be the basis function. When $M$ is fixed, we can choose $N$ (the number of time steps in forward pass) as $kM$, such as $k=2$, so that the forward ODEs \eqref{char} and \eqref{rhos} can be solved accurately.
Then, the parameters $\theta$ in the neural network can be optimized by some popular optimizor, such as SGD, ADAM, BFGS and so on.

Next, to demonstrate the effective of the above network design, we compare it experimentally with the following network structure:
$$
\boldsymbol{v}^*(x,t;\theta)=\sum_{l=1}^L[W_2^{(l)}(t)\sigma(W_1^{(l)}(t)x + b_1^{(l)}(t))+b_2^{(l)}(t)],
$$
where $W_1^{(l)}(t) \in \mathbb{R}^{H\times d}, W_2^{(l)}(t)\in \mathbb{R}^{d\times H}, b_1^{(l)}(t)\in \mathbb{R}^H$ and $b_2^{(l)}(t)\in \mathbb{R}^d$ are represented by the nodal basis functions, i.e.
\begin{align*}
W_1^{(l)}(t) &= \sum_{i=0}^M W_{1i}^{(l)} \phi_i(t),\\
W_2^{(l)}(t) &= \sum_{i=0}^M W_{2i}^{(l)} \phi_i(t),\\
b_1^{(l)}(t) &= \sum_{i=0}^M b_{1i}^{(l)} \phi_i(t),\\
b_2^{(l)}(t) &= \sum_{i=0}^M b_{2i}^{(l)} \phi_i(t).
\end{align*}

We have found that these two velocity fields $\boldsymbol{v}(x,t;\theta)$ and $\boldsymbol{v}^*(x,t;\theta)$ have different network structures, however, the same number of parameters, $L(M+1)(2dH+H+d)$. Therefore, in order to compare these two neural network's architecture fairly and intuitively, we give an example in the 1-dimensional case ($d=1$) for Gaussian problem. The initial density $\rho_0$ is a Gaussian with means $0$ and variance $0.3$, while the target density $\rho_1$ is a Gaussian with means $-4$ and variance $1.0$.
The parameters of the network structure are chosen as $L = 1, M = 5$ and $H=1$ for both velocity fields. 
We train our networks using 4000 iterations of Adam with a learning rate of $0.01$. 
We visualize the trained velocity field $\boldsymbol{v}(x,t;\theta)$ and $\boldsymbol{v}^*(x,t;\theta)$ at $x=-4,0,2$ in Figure \ref{v}. It can be observed that the oscillation of velocity field $\boldsymbol{v}$ in the time direction is obviously smaller than that of the velocity field $\boldsymbol{v}^*$, both in terms of frequency and amplitude. 
The frequency of $\boldsymbol{v}$ is exactly 5, which is actually equal to $M$ and clearly smaller than the frequency of the velocity field $\boldsymbol{v}^*$. 
In addition, the maximum oscillation amplitude of $\boldsymbol{v}$ is about 5.5, while the maximum oscillation amplitude of $\boldsymbol{v}^*$ is about 16.

\begin{figure}[H]

\begin{minipage}[c]{.05\textwidth}
$\boldsymbol{v}$
\end{minipage}
\begin{minipage}[c]{1.50\textwidth}
\includegraphics[width=4cm]{images/velocity/v(-4).png}
%\includegraphics[width=3.5cm]{images/velocity/v(-2).png}
\includegraphics[width=4cm]{images/velocity/v(0).png}
\includegraphics[width=4cm]{images/velocity/v(2).png}
\end{minipage}

\begin{minipage}[c]{.05\textwidth}
$\boldsymbol{v}^*$
\end{minipage}
\begin{minipage}[c]{1.50\textwidth}
\includegraphics[width=4cm]{images/velocity/v2(-4).png}
%\includegraphics[width=2.5cm]{images/crowd motion/crowd2_d2_true.png}
\includegraphics[width=4cm]{images/velocity/v2(0).png}
\includegraphics[width=4cm]{images/velocity/v2(2).png}
\end{minipage}
\caption{The comparison of network structures $\boldsymbol{v}$ and $\boldsymbol{v}^*$.}
\label{v}
\end{figure}

\subsection{Crowd motion}
Our method can also be easily applied to the crowd motion problem\cite{Ruthotto9183}. In contrast to the OT problem, the crowd motion problem not only needs to move the  initial  density $\rho_{0}$ approximately to the  target density $\rho_{1}$, but also  expects to avoid some obstacles in the dynamic movement. The obstacles can be expressed by introducing an added term to the loss function, i.e.  the preference term:
$$
\mathcal{Q}(\rho) = \int_0^1\int_{\mathbb{R}^d} Q(x)\rho(x,t)\mathrm{d}x \mathrm{d}t
$$
where $Q:\mathbb{R}^d  \rightarrow \mathbb{R}$, models the spatial preferences of agents, the larger $Q(x)$ is, the closer the position of $x$ is to the obstacles. We can get the following formulation:
\begin{align*}
    \min_{(\boldsymbol{v},\rho) \in \mathcal{C}(\rho_0,\rho_1)}\mathcal{F}_{cm}(\boldsymbol{v},\rho) := \mathcal{E}(\boldsymbol{v},\rho)  + \mathcal{Q}(\rho)
\end{align*}
It shows that the crowd motion problem is the specific case of MFP for $L(\rho,\boldsymbol{v})=\rho|\boldsymbol{v}|^2+Q\rho$ and $\mathcal{F}=0$.
The method to solve the crowd motion problem is almost the same as the OT problem. Firstly, as in section 2.1, we relax the terminal density as an implicit condition penalized by KL divergence term $\mathcal{P}$ to get the following problem:
\begin{align}\label{rcrm}
    \min_{(\boldsymbol{v},\rho) \in \mathcal{C}(\rho_0)} \mathcal{E}(\boldsymbol{v},\rho)  + \mathcal{Q}(\rho) +\mathcal{P}(\rho)
\end{align}
Then we adopt the Lagrangian discretization method presented in section 2.2 to get the   semi-discrete formulation of \eqref{rcrm}
\begin{align}\label{semcd}
    \min_{\boldsymbol{v} }\overline{\mathcal{E}} (\boldsymbol{v},\rho)  + 
 \overline{\mathcal{P}} (\rho) + \overline{\mathcal{Q}} (\rho)
\end{align}
s.t.
\begin{equation*}  
\left\{  
    \begin{aligned} 
 &\frac{\mathrm{d}}{\mathrm{d}t}\mathbf{z}(x_i,t)=\boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mathbf{z}(x_i,0)=x_i, ~x_i \sim \mu_0(x_{i}) \\
 &\frac{\mathrm{d}}{\mathrm{d}t}\rho(\mathbf{z}(x_i,t),t)=-\rho(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\rho(\mathbf{z}(x_i,0),0)=\rho_0(x_i)\\
 &\frac{\mathrm{d}}{\mathrm{d}t}\mu(\mathbf{z}(x_i,t),t)=-\mu(\mathbf{z}(x_i,t),t)\nabla \cdot \boldsymbol{v}(\mathbf{z}(x_i,t),t),~\mu(\mathbf{z}(x_i,0),0)=\mu_0(x_i)  
\end{aligned}  
\right.  
\end{equation*} 
where $\overline{\mathcal{E}}, \overline{\mathcal{P}}$ are defined in \eqref{disE},\eqref{disP} respectively. $\overline{\mathcal{Q}}$ is the discrete version of $\mathcal{Q}$:
\begin{align*}
    \overline{\mathcal{Q}} (\rho)&:= \int_0^1 \sum_{i=1}^r w_i(t)Q(\mathbf{z}(x_i,t)) \mathrm{d}t
\end{align*}
The  velocity  field $v$ is parameterized by neural network $v(x,t;\theta)$,  and we use composite Simpson formula to discrete \eqref{semcd} so that backpropagation can be used to calculate the gradient. 

